On the impact of numerology in NR V2X Mode 2 with sensing and no-sensing resource selection

In this paper, we use a New Radio (NR) Vehicular-to-everything (V2X) standard compliant simulator based on ns-3, to study the impact of NR numerologies on the end-to-end performance. In particular, we focus on NR V2X Mode 2, used for autonomous resource selection in out-of-coverage communications, and consider the two key procedures defined in 3GPP: sensing and non-sensing based resource selection. We pay particular attention to the interplay between the operational numerology and the resource selection window length, a key parameter of NR V2X Mode 2. The results in a standard-compliant, end-to-end simulation platform show that in all cases, for basic service messages, a higher numerology is beneficial because of different reasons, depending on the way the resource selection window length is established.

==> feature_table.tex <==
% \begin{table*}[!t]
% %\small
% \caption{List of measurements from LTE protocol stack used to create the dataset}
% \label{table_input_features}
% \centering
% \begin{tabular}{|>{\columncolor[gray]{0.95}}p{0.35\textwidth}|>{\columncolor[gray]{0.95}}p{0.4\textwidth}|}
% \hline
% \rowcolor[gray]{0.90}\textbf{Layer}     & \textbf{Measurements} \\
% \hline
% \multicolumn{2}{|c|}{\textbf{Input features}}
% \\
% \hline
% Application & 1. Throughput UL \newline 2. Average number of received packets UL \newline 3. Average number of received bytes UL \newline 4. Throughput DL \newline 5. Average number of received packets DL \newline 6. Average number of received bytes DL \\
% \hline
% RRC & 7. Cell ID of serving cell \newline 8. RSRP from serving cell \newline 9. RSRQ from serving cell \newline 10. Cell ID of neighbour 1 \newline 11. RSRP from neighbour 1 \newline 12. RSRQ from neighbour 1  \newline \hspace*{1cm} \textbf{. . . . .}  \newline 31. Cell ID of neighbour 8 \newline 32. RSRP from neighbour 8 \newline 33. RSRQ from neighbour 8 \newline 34. Total number of radio link failures \newline 35. Total number of handovers \newline 36. First target cell ID to handover
% \\
% \hline
% PDCP & 37. Total number of transmitted PDCP PDUs DL \newline 38. Total number of received PDCP PDUs DL \newline 39. Total bytes transmitted DL \newline 40. Average PDCP PDU delay DL \newline 41. Minimum value of the PDCP PDU delay DL \newline 42. Maximum value of the PDCP PDU delay DL \newline 43. Minimum PDCP PDU size DL \newline 44. Maximum PDCP PDU size DL \newline 45. Total number of transmitted PDCP PDUs UL \newline 46. Total number of received PDCP PDUs UL \newline 47. Total bytes transmitted UL \newline 48. Average PDCP PDU delay UL \newline 49. Minimum value of the PDCP PDU delay UL \newline 50. Maximum value of the PDCP PDU delay UL \newline 51. Minimum PDCP PDU size UL \newline 52. Maximum PDCP PDU size UL
% \\
% \hline
% RLC & 53. Total number of transmitted RLC PDUs DL \newline 54. Total number of received RLC PDUs DL \newline 55. Total number of bytes transmitted DL \newline 56. Total number of bytes received DL \newline 57. Average RLC PDU delay DL \newline 58. Minimum value of the RLC PDU delay DL \newline 59. Maximum value of the RLC PDU delay DL \newline 60. Minimum RLC PDU size DL \newline 61. Maximum RLC PDU size DL \newline 62. Total number of transmitted RLC PDUs UL \newline 63. Total number of received RLC PDUs UL \newline 64. Total bytes transmitted RLC PDUs UL \newline 65. Total bytes received RLC PDUs UL \newline 66. Average RLC PDU delay UL \newline 67. Minimum value of the RLC PDU delay UL \newline 68. Maximum value of the RLC PDU delay UL \newline 69. Minimum RLC PDU size UL \newline 70. Maximum RLC PDU size UL
% \\
% \hline
% MAC & 71. Initial MCS \newline 72 Average TB size UL \newline 73. Average TB size DL \newline 74. Average MCS UL \newline 75. Average MCS DL \newline 76. Average RB occupied UL \newline 77. Average RB occupied DL \newline 78. DL CQI inband \newline 79. DL CQI wideband \newline 80. UL CQI
% \\
% \hline
% PHY & 81. Average SINR DL \newline 82. Average SINR UL \newline 83. Average number of DL HARQ NACKs \newline 84. Average number of UL HARQ NACKs
% \\
% % \hline
% % Key RRC and MAC KPIs for multiple use case & 83. First target cell id to handover  \newline 84. Initial MCS
% % \\
% \hline
% % \multicolumn{2}{|c|}{\textbf{Output feature}}
% % \\
% % \hline
% {\textbf{Output feature}} & 1. File download time (sec) [Application]
% \\
% \hline
% \end{tabular}
% \end{table*}


% %\newline \hspace*{1cm} \textbf{.} \newline \hspace*{1cm} \textbf{.}


% New Table

\begin{table*}
%\renewcommand{\arraystretch}{1.3}
\caption{List of measurements from LTE protocol stack used to create the dataset}
\label{table_input_features}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|m{0.7cm}||m{5.3cm}|m{5.0cm}|m{5.0cm}|}
%\begin{tabular}{|c||c|c|c|}
\hline
\multicolumn{4}{|c|}{\cellcolor[HTML]{C0C0C0}Input feature} \\ \hline
Layer & \multicolumn{3}{c|}{Measurements} \\

\hline
APP & \begin{tabular}[c]{@{}l@{}}1. Throughput UL\\ 5. Avg. number of rcvd packets DL\end{tabular} & \begin{tabular}[c]{@{}l@{}}2. Avg. number of rcvd packets UL\\ 4. Throughput DL\end{tabular} & \begin{tabular}[c]{@{}l@{}}3. Avg. number of rcvd bytes UL\\ 6. Avg. number of rcvd bytes DL\end{tabular} \\

\hline

RRC & \begin{tabular}[c]{@{}l@{}}7. Cell ID of serving cell\\ 10. Cell ID of neighbour 1\\ \hspace*{1cm} \textbf{.}\\ \hspace*{1cm} \textbf{.}\\ 31. Cell ID of neighbour 8\\ 34. Total number of radio link failures\end{tabular} & \begin{tabular}[c]{@{}l@{}}8. RSRP from serving cell\\ 11. RSRP from neighbour 1\\ \hspace*{1cm} \textbf{.}\\ \hspace*{1cm} \textbf{.}\\ 32. RSRP from neighbour 8\\ 35. Total number of handovers\end{tabular} & \begin{tabular}[c]{@{}l@{}}9. RSRQ from serving cell\\ 12. RSRQ from neighbour 1\\ \hspace*{1cm} \textbf{.}\\\hspace*{1cm} \textbf{.}\\ 33. RSRQ from neighbour 8\\ 36. First target cell ID to handover\end{tabular} \\
\hline

PDCP & \begin{tabular}[c]{@{}l@{}}37. Total number of txed PDCP PDUs DL\\ 40. Avg. PDCP PDU delay DL\\ 43. Min. PDCP PDU size DL\\ 46. Total number of rcvd PDCP PDUs UL\\ 49. Min. value of the PDCP PDU delay UL\\ 52. Max. PDCP PDU size UL\end{tabular} & \begin{tabular}[c]{@{}l@{}}38. Total number of rcvd PDCP PDUs DL\\ 41. Min. value of the PDCP PDU delay DL\\ 44. Max. PDCP PDU size DL\\ 47. Total bytes txed UL\\ 50. Max. value of the PDCP PDU delay UL\end{tabular} & \begin{tabular}[c]{@{}l@{}}39. Total bytes txed DL\\ 42. Max. value of the PDCP PDU delay DL\\ 45. Total number of txed PDCP PDUs UL\\ 48. Avg. PDCP PDU delay UL\\ 51. Min. PDCP PDU size UL\end{tabular} \\ 
\hline

RLC & \begin{tabular}[c]{@{}l@{}}53. Total number of txed RLC PDUs DL\\ 56. Total number of bytes received DL\\ 59. Max. value of the RLC PDU delay DL\\ 62. Total number of txed RLC PDUs UL\\ 65. Total bytes rcvd RLC PDUs UL\\ 68. Max. value of the RLC PDU delay UL\end{tabular} & \begin{tabular}[c]{@{}l@{}}54. Total number of rcvd RLC PDUs DL\\ 57. Avg. RLC PDU delay DL\\ 60. Min. RLC PDU size DL\\ 63. Total number of rcvd RLC PDUs UL\\ 66. Avg. RLC PDU delay UL\\ 69. Minimum RLC PDU size UL\end{tabular} & \begin{tabular}[c]{@{}l@{}}55. Total number of bytes txed DL\\ 58. Min. value of the RLC PDU delay DL\\ 61. Max. RLC PDU size DL\\ 64. Total bytes txed RLC PDUs UL\\ 67. Min. value of the RLC PDU delay UL\\ 70. Maximum RLC PDU size UL\end{tabular} \\
\hline

MAC & \begin{tabular}[c]{@{}l@{}}71. Initial MCS\\ 74. Avg. MCS UL\\ 77. Avg. RB occupied DL\\ 80. UL CQI\end{tabular} & \begin{tabular}[c]{@{}l@{}}72 Avg. TB size UL\\ 75. Avg. MCS DL\\ 78. DL CQI inband\end{tabular} & \begin{tabular}[c]{@{}l@{}}73. Avg. TB size DL\\ 76. Avg. RB occupied UL\\ 79. DL CQI wideband\end{tabular} \\
\hline

PHY & \begin{tabular}[c]{@{}l@{}}81. Avg. SINR DL\\ 84. Avg. number of UL HARQ NACKs\end{tabular} & 82. AVG. SINR UL & 83. Avg. number of DL HARQ NACKs \\
\hline

\multicolumn{4}{|c|}{\cellcolor[HTML]{C0C0C0}Output feature} \\ \hline
APP & \multicolumn{3}{l|}{1. File download time {[}sec{]}} \\ \hline
\end{tabular}}
\end{table*}


